WeaverBird: Empowering Financial Decision-Making with Large Language Model, Knowledge Base, and Search Engine

We present WeaverBird, an intelligent dialogue system designed specifically for the finance domain. Our system harnesses a large language model of GPT architecture that has been tuned using extensive corpora of finance-related text. As a result, our system possesses the capability to understand complex financial queries, such as "How should I manage my investments during inflation?", and provide informed responses. Furthermore, our system incorporates a local knowledge base and a search engine to retrieve relevant information. The final responses are conditioned on the search results and include proper citations to the sources, thus enjoying an enhanced credibility. Through a range of finance-related questions, we have demonstrated the superior performance of our system compared to other models. To experience our system firsthand, users can interact with our live demo at https://weaverbird.ttic.edu, as well as watch our 2-min video illustration at https://www.youtube.com/watch?v=yofgeqnlrMc.

==> font/texmf/doc/fonts/hbf/ksc5601/hanja65/README <==
This is the README file of the hanja65.tar.gz package. 

It contains a Korean hanja bitmap file (*no* hangul!) together with
its HBF header file, an hbf2gf configuration file and .tfm files to be
used with the CJK package for LaTeX2e.

The package follows the TDS directory structure.

Please read the documentation (especially the INSTALL file) of CJK for
further details.

[Note: Be warned that if you select \CJKhanja and use this font for
       hangul syllables you will get wrong characters without an error
       message! Solution: use \CJKhangul.]

---End of README---

